Deviations from He I Case B Recombination Theory and Extinction Corrections in the Orion Nebula

We are engaged in a comprehensive program to find reliable elemental abundances in and to probe the physical structure of the Orion Nebula, the brightest and best-resolved H II region. In the course of developing a robust extinction correction covering our optical and ultraviolet FOS and STIS observations, we examined the decrement within various series of He I lines. The decrements of the 2^3S-n^3P, 2^3P-n^3S and 3^3S-n^3P series are not in accord with caseB recombination theory. None of these anomalous He I decrements can be explained by extinction, indicating the presence of additional radiative transfer effects in He I lines ranging from the near-IR to the near-UV. CLOUDY photoionization equilibrium models including radiative transfer are developed to predict the observed He I decrements and the quantitative agreement is quite remarkable. Following from these results, select He I lines are combined with H I and [O II] lines and stellar extinction data to validate a new normalizable analytic expression for the wavelength dependence of the extinction. In so doing, the He+/H+ abundance is also derived.

==> response <==
RE: ApJ Submission MS# 70035

Dear Eric Herbst,

Thank you for again passing on the referee's comments.  I hope that I have
addressed the one issue s/he still had with the paper.  I have attached my
response (indented) below.

Thank you
Kevin Blagrave
University of Toronto

I have only one criticism.  Regarding the last paragraph of page 13, I am
still confused.  First, I think the first sentence is much too long.
Second, I still don't understand why the authors are surprised that the
3188 ratios plotted in figures 2a and 2b of Benjamin et al. 1999 are near
unity.  Benjamin et al. did not include radiative transfer effects.  This
means that the predicted values are likely too high, and the plotted
I_obs/I_predicted ratios are therefore too low.  But there is also the
apparent trend shortward of 3820 that shifts the plotted ratios upwards.
This effect has the opposite sign of the effect of neglecting radiative
transfer, so that the two effects cancel out somewhat (although admittedly
one would not expect a priori that they would cancel out so perfectly).
The lack of radiative transfer effects in the Benjamin et al. predictions
might be the only reason that the upward trend does not appear to apply to
3188.  The paragraph would be much more clear with something like the
following:

The observed intensity of 3188 may be strongly self-absorbed, but this
effect is not included in the Benjamin et al. predictions.  Inclusion of
the effect would cause the plotted 3188 ratios to increase, possibly
enough to agree with the apparent upward trend of the other lines
shortward of 3820.

        Thanks again.  I realize that our point must not have been very
        well communicated.  Sorry about that.  I think it is addressed
        more clearly here.  (I have shortened the long sentence too.)
        The point is that the upward trend cannot be explained by
        the inclusion of radiative transfer, as was suggested in
        BSS.

        Changed paragraph on page 13:

        "In comparing their case~B results with the OTV92
        observations, \citet{ben99} noted (their Figs.~2a and 2b) that the lines
        (singlets and triplets) shortward of $\lambda$3820 were consistently
        brighter than predicted, increasingly with decreasing wavelength, 
        except $\lambda$3188 which appeared to be accurately predicted.
        They suggested that the upward trend shortward of $\lambda$3820
        could be due to unaccounted for
        radiative transfer effects, though this seems very unlikely given the
        lines involved.
        Inclusion of radiative transfer (see discussion below) would
        cause the plotted $\lambda$3188 ratios to increase --
        possibly enough to
        agree with the apparent upward trend shortward
        of $\lambda$3820 --
        while not affecting the other lines shortward of $\lambda$3820.  
        If alternatively this upward trend arose..."



